Neural Radiosity

We introduce Neural Radiosity, an algorithm to solve the rendering equation by minimizing the norm of its residual similar as in traditional radiosity techniques. Traditional basis functions used in radiosity techniques, such as piecewise polynomials or meshless basis functions are typically limited to representing isotropic scattering from diffuse surfaces. Instead, we propose to leverage neural networks to represent the full four-dimensional radiance distribution, directly optimizing network parameters to minimize the norm of the residual. Our approach decouples solving the rendering equation from rendering (perspective) images similar as in traditional radiosity techniques, and allows us to efficiently synthesize arbitrary views of a scene. In addition, we propose a network architecture using geometric learnable features that improves convergence of our solver compared to previous techniques. Our approach leads to an algorithm that is simple to implement, and we demonstrate its effectiveness on a variety of scenes with non-diffuse surfaces.

==> materials_fig.tex <==
\newcommand\ballwidth{0.17}
\newcommand\ballmapeoffset{15pt}

\begin{figure*}[ht]
  \centering
    
    \makebox[0pt]{\rotatebox{90}{\hspace{35pt} LHS}}
    \includegraphics[width=\ballwidth\textwidth]{NNMitsuba Paper/Renderings/Balls/mat-diffuse-mlp-spp16-m1.png}
    \includegraphics[width=\ballwidth\textwidth]{NNMitsuba Paper/Renderings/Balls/mat-textured-mlp-spp16-m1.png}
    \includegraphics[width=\ballwidth\textwidth]{NNMitsuba Paper/Renderings/Balls/mat-plasbeck-mlp-spp16-m1.png}
    \includegraphics[width=\ballwidth\textwidth]{NNMitsuba Paper/Renderings/Balls/mat-nopreserve-mlp-spp16-m1.png}
    \includegraphics[width=\ballwidth\textwidth]{NNMitsuba Paper/Renderings/Balls/mat-coppermlp-spp16-m1.png}

    \vspace{-10pt}    
    \hspace{\ballmapeoffset}
    \makebox[0pt]{{MAPE:}}
    \hspace{-\ballmapeoffset}
    \makebox[\ballwidth\textwidth]{{0.020}}
    \makebox[\ballwidth\textwidth]{{0.022}}
    \makebox[\ballwidth\textwidth]{{0.047}}
    \makebox[\ballwidth\textwidth]{{0.042}}
    \makebox[\ballwidth\textwidth]{{0.038}}

    \makebox[0pt]{\rotatebox{90}{\hspace{35pt} RHS}}
    \includegraphics[width=\ballwidth\textwidth]{NNMitsuba Paper/Renderings/Balls/mat-diffuse-rhs-spp16-m16.png}
    \includegraphics[width=\ballwidth\textwidth]{NNMitsuba Paper/Renderings/Balls/mat-textured-rhs-spp16-m16.png}
    \includegraphics[width=\ballwidth\textwidth]{NNMitsuba Paper/Renderings/Balls/mat-plasbeck-rhs-spp16-m16.png}
    \includegraphics[width=\ballwidth\textwidth]{NNMitsuba Paper/Renderings/Balls/mat-nopreserve-rhs-spp16-m16.png}
    \includegraphics[width=\ballwidth\textwidth]{NNMitsuba Paper/Renderings/Balls/mat-copper-rhs-spp16-m16.png}

    \vspace{-10pt}
    \hspace{\ballmapeoffset}
    \makebox[0pt]{{MAPE:}}
    \hspace{-\ballmapeoffset}
    \makebox[\ballwidth\textwidth]{{0.018}}
    \makebox[\ballwidth\textwidth]{{0.019}}
    \makebox[\ballwidth\textwidth]{{0.021}}
    \makebox[\ballwidth\textwidth]{{0.021}}
    \makebox[\ballwidth\textwidth]{{0.021}}

    \makebox[0pt]{\rotatebox{90}{\hspace{30pt} Residual}}
    \includegraphics[width=\ballwidth\textwidth]{NNMitsuba Paper/Renderings/Balls/mat-diffuse-residual-spp16-m16.png}
    \includegraphics[width=\ballwidth\textwidth]{NNMitsuba Paper/Renderings/Balls/mat-textured-residual-spp16-m16.png}
    \includegraphics[width=\ballwidth\textwidth]{NNMitsuba Paper/Renderings/Balls/mat-plasbeck-residual-spp16-m16.png}
    \includegraphics[width=\ballwidth\textwidth]{NNMitsuba Paper/Renderings/Balls/mat-nopreserve-residual-spp16-m16.png}
    \includegraphics[width=\ballwidth\textwidth]{NNMitsuba Paper/Renderings/Balls/mat-copper-residual-spp16-m16.png}
    
    \vspace{-10pt}    
    \makebox[0pt]{\rotatebox{90}{\hspace{35pt} Truth}}
    \includegraphics[width=\ballwidth\textwidth]{NNMitsuba Paper/Renderings/Balls/mat-diffuse-int-scene-spp256-m1.png}
    \includegraphics[width=\ballwidth\textwidth]{NNMitsuba Paper/Renderings/Balls/mat-textured-int-scene-spp256-m1.png}
    \includegraphics[width=\ballwidth\textwidth]{NNMitsuba Paper/Renderings/Balls/mat-plasbeck-int-scene-spp256-m1.png}
    \includegraphics[width=\ballwidth\textwidth]{NNMitsuba Paper/Renderings/Balls/mat-nopreserve-int-scene-spp256-m1.png}
    \includegraphics[width=\ballwidth\textwidth]{NNMitsuba Paper/Renderings/Balls/mat-copper-int-scene-spp256-m1.png}
    
    \makebox[\ballwidth\textwidth]{{Diffuse}}
    \makebox[\ballwidth\textwidth]{{Textured Diffuse}}
    \makebox[\ballwidth\textwidth]{{Rough Plastic}}
    \makebox[\ballwidth\textwidth]{{Textured Rough Plastic}}
    \makebox[\ballwidth\textwidth]{{Rough Copper}}

    
%    \subcaptionbox{\label{third-subfig}}{%
%     \includegraphics[width=0.15\textwidth]{coppertestmlp-spp8-m1-square.png}
%  }

    \caption{Our Neural Radiosity approach tested on various BSDFs. The materials range from prefect diffuse surfaces where the outgoing radiance is constant in all directions $\omega$ over the unit hemisphere, to moderately specular conductor and plastic materials. The rough surfaces here follow the Beckmann distribution for the microfacet component with roughness = 0.1.}

  \label{fig:materials}
\end{figure*}


==> scratch.tex <==
\appendix
\section{Timing Experiments}

\begin{figure*}[hbt]
  \centering
  \subcaptionbox{Equal rendering time of 14 seconds. \label{fig:LHS_time}}{%
\includegraphics[width = 0.48\textwidth]{NNMitsuba Paper/Figs/LHS-timing.pdf}
  }
  \subcaptionbox{Equal rendering time of 3.5 minutes \label{fig:RHS_time}}{%
    \includegraphics[width = 0.48\textwidth]{NNMitsuba Paper/Figs/RHS-timing.pdf}
  }
  \caption{Timing studies given a pre-trained model}
  \label{fig:timing_study}
\end{figure*}



\section{Ablation Studies}
\section{Multi-resolution grids}


\begin{figure*}[hbt]
  \centering
  \subcaptionbox{Increasing the resolution level in a multi-resolution setting. \label{fig:multi_res}}{%
\includegraphics[width = 0.48\textwidth]{NNMitsuba Paper/Figs/MultiRes.pdf}
  }
  \subcaptionbox{Single-Resolution vs. Multi-Resolution training. \label{fig:single_res}}{%
    \includegraphics[width = 0.48\textwidth]{NNMitsuba Paper/Figs/SingleVsMultiRes.pdf}
  }
  \caption{Resolution impact on LHS renderings}
  \label{fig:Res_study}
\end{figure*}




\section{Complementary Scenes}


\begin{figure*}[hbt]
  \centering

\includegraphics[width = 0.48\textwidth]{NNMitsuba Paper/Renderings/Bedroom/bedroommlp-spp16-m1.jpg}
\includegraphics[width = 0.48\textwidth]{NNMitsuba Paper/Renderings/Bedroom/bedroomrhs-spp16-m32.jpg}
\includegraphics[width = 0.48\textwidth]{NNMitsuba Paper/Renderings/Bedroom/bedroomGTint-scene-spp512-m1.jpg}
\includegraphics[width = 0.48\textwidth]{NNMitsuba Paper/Renderings/Bedroom/bedroomresidual-abs-spp16-m32.jpg}

  \caption{Complementary Scenes}
  \label{fig:Complementary_scenes}
\end{figure*}


==> veach_training_fig.tex <==
\begin{figure*}[ht]
    \centering
    \includegraphics[width = \textwidth]{NNMitsuba Paper/Figs/Training_veach.pdf}
    \caption{Training milestones for the \emph{Veach Door} Scene. RHS, LHS, and the relative residual for certain training steps are visualized. As training proceeds, the LHS gradually learns the radiance distribution. As a result, the light coming from the room behind the door propagates to the RHS renderings. Note that the residual visualisations here are the relative residual. The batch size(N) is 8192, M is 32, and 48K steps(S) were used. Thus, the total number of samples(N $\times$ M $\times$ S) used here is 12580 M.  }
    \label{fig:veach_training_milestones}
\end{figure*}


\begin{figure}[h]
    \centering
    \subcaptionbox{}{
        \includegraphics[width = 0.47\columnwidth]{NNMitsuba Paper/Figs/ImageBaseError.pdf}
    }
    \subcaptionbox{}{
        \includegraphics[width = 0.48\columnwidth]{NNMitsuba Paper/Figs/VeachTrainingCurve.pdf}
    }
    \caption{(a) Image-based MSE of RHS/LHS with the path-tracing ground truth. Note that the vertical axis is log-scale to show the two curves distinctively. As the chart illustrates, the RHS is always more faithful to the ground truth compared to the LHS. This is because RHS involves one step of ray tracing that integrates multiple network outputs, as opposed to the LHS which computes one network output per sample. (b) Relative residual loss curve during training of the \emph{Veach Door} scene. The milestones marked on the line chart correspond to the training steps visualized in Figure~\ref{fig:veach_training_milestones}.\label{fig:veach_training_charts}}
\end{figure}


